Rational Homotopy Type of Complements of Submanifold Arrangements

In this work we provide an explicit cdga that controls the rational homotopy type of the complement $X-\cup_i Z_i$, where $X$ is a smooth compact algebraic variety and $\{Z_i\}$ is a collection of subvarieties such that all set-theoretical intersections are smooth. The model is given in terms of the cohomology of all intersections of $Z_i$'s, and the natural maps induced by the inclusions. Our construction is inspired by the work of J.Morgan, who covered the fundamental case where $\{Z_i\}$ is a divisor with normal crossings, and it is built on developments of the theory of mixed Hodge diagrams by Cirici-Horel. We avoid any explicit reduction to the normal crossings divisor case, e.g. via the wonderful compactification of De Concini-Procesi. As an application of our approach we recover and generalize a few separate results on the complements of arrangements in a uniform manner. These include the Kritz-Totaro model for graph configuration spaces, Yuzvinsky's model for affine subspace arrangements and Dupont's model for complements of hypersurfaces with hyperplane-like intersection.

==> lattice_colattice.tex <==
\stoptoc
In this section, and in it only we change our notation for intersection posets 
to make it easier to relate our work to the works \cite{To},\cite{Petersen} and \cite{DSY}
where certain spectral sequences related to arrangements are studied.
Our goal is to provide a uniform description of these constructions.
Working additively we will use the framework of homotopical algebra over 
posets. The exposition is independent of our previous setup.
The construction of lattice spectral sequences here follows 
\cite{To},\cite{Petersen}
quite closely, 
while our colattice spectral sequence described below
is less restrictive than the original construction from \cite{DSY}
applied to the case of arrangements of closed subspaces.

Let $X$ be a topological space, and $(L,\le)$ be the intersection 
poset of an arrangement
$L_x\subset X$ of closed subspaces ordered by inclusion: 
$x\le y\iff L_x\subseteq L_y$. 
Denote the unique maximal element of $L$ by $1$, so $L_1=X$.
Let $r\colon L\ar \mathbb{Z}$ be a (weak) rank function, i.e. $r(x)<r(y)$ if $x<y$.
We let $i_x\colon L_x\ar X$ be the inclusion of the subspace, and set $j_x\colon L_x-\cup_{y<x}L_y\ar X$ to be
the inclusion of the stratum corresponding to $x\in L$.
Here $j:=j_1$ is the inclusion of the complement of the arrangement.

In what follows, a sheaf is understood to be a sheaf of abelian groups.
Working additively we often consider sheaves as objects in the derived category.
We use the cohomological grading notation throughout.

Let $\mc{L}\in \Ch(\Sh_U)$ be a complex of sheaves on $U$.
Then $\mc{L}=j^*\tilde{\mc{L}}$
for some $\tilde{\mc{L}}\in\Ch(\Sh_X)$ (e.g.\ $\tilde{\mc{L}}=j_*\mc{L}$).
Our aim is to construct two spectral sequences converging to 
$\mb{H}^*(U;\mc{L})\simeq \mb{H}^*(X;Rj_*\mc{L})$.
%The Leray spectral sequence is associated with the canonical filtration $\tau^{\le}$ on $Rj_*\mc{L}$.
To this end we will describe two filtrations on $Rj_* \mc{L}$ reflecting the combinatorics of $(L,\le)$.
We refer to the corresponding spectral sequences ${}_{L}E_1$ and ${}^{L}E_2$, 
as the \emph{lattice} and the
\emph{colattice} spectral sequences respectively.
The former was introduced and studied in additive setting independently by 
Tosteson \cite{To} and Petersen \cite{Petersen}.
It allows one, for example, 
to deduce the Goresky-MacPherson formula \ref{eq:gormac} 
in a straightforward way.
The latter was developed by 
Denham-Suciu-Yuzvinsky \cite{DSY} in order to establish vanishing results for 
local systems on certain arrangement complements.

As a motivation consider an arrangement given by one subspace 
$i\colon L_0\ar L_1$.

1. In this case the \emph{lattice} spectral sequence originates from the triangle:
$$i_*Ri^!\ar \id_X \ar Rj_*j^*\ar.$$
Namely, if $\mc{L}=j^*\tilde{\mc{L}}$ for some $\tilde{\mc{L}}\in \Ch(\Sh_X)$, substituting
$\tilde{\mc{L}}$ followed by $R\Gamma(-)$ gives the triangle 
$$R\Gamma(i^!\tilde{\mc{L}})\ar R\Gamma(\tilde{\mc{L}})\ar R\Gamma(Rj_*\mc{L})\ar,$$
which gives us thte long exact sequence of the cohomology groups
$$\ar \mb{H}^k_{L_0}(L_1;\tilde{\mc{L}}) \ar \mb{H}^k(L_1;\tilde{\mc{L}})\ar \mb{H}^k(U;\mc{L}) \ar 
\mb{H}^{k+1}_{L_0}(L_1;\tilde{\mc{L}})\ar,$$
where by definition $\mb{H}^{*}_{L_0}(L_1;\tilde{\mc{L}})=\mb{H}^{*}(L_0;Ri^!\tilde{\mc{L}})$
is the cohomology of the derived complex of sections of $\tilde{\mc{L}}$ supported on $L_0$.
Observe that in the case $\tilde{\mc{L}}=Rj_*\mc{L}$ the third arrow is an isomorphism and 
one gets no additional information.

Thus, in the case of the lattice spectral sequence it is important to work with 
$\tilde{\mc{L}}\in \Ch(\Sh_X)$,
and not with its restriction $\mc{L}$. 
Some natural variants also might be useful, for example one can take $\tilde{\mc{L}}$ to be $j_!\mc{L}$ or 
the non derived $j_*\mc{L}$ if
$\mc{L}$ was a local system.
We are particularly interested in the case when $\tilde{\mc{L}}=j_*\mc{L}$ is a local system.
In this case the long exact sequence relates $H^*(U;j^*\tilde{\mc{L}})$ with 
$H^*_{L_0}(L_1;\tilde{\mc{L}})$ and $H^*(L_1;\tilde{\mc{L}})$.
Moreover, in the algebraic setting, assuming $\tilde{\mc{L}}$ is unitary and the arrangement is smooth and compact, 
the terms of the lattice spectral sequence are pure Hodge structures, which is useful 
for proving degeneration properties of the spectral sequence.

2. The colattice spectral sequence requires a bit more work. Starting with the dual triangle
$$j_!j^*\ar \id_X \ar i_*i^*\ar,$$
and applying it to $Rj_*\mc{L}$ we get
$$j_! \mc{L}\ar Rj_*\mc{L}\ar i_*i^*Rj_*\mc{L}\ar .$$
Applying $R\Gamma$ and passing to the cohomology we obtain a long exact sequence 
$$\ar \mb{H}^k(L_1,L_0;\mc{L})\ar \mb{H}^k(U;\mc{L})\ar \mb{H}^k(L_1;i^*Rj_*\mc{L})\ar .$$
Here by definition $\mb{H}^k(L_1,L_0;\mc{L})=\mb{H}^k(L_1;j_!\mc{L})$, and in the case $L_1$ is compact
it is equal to $\mb{H}^k_c(U;\mc{L})$. Note that $\mb{H}^k(L_1;i^*Rj_*\mc{L})$ 
is equal to $\mb{H}^*(V-L_1;j'^*\mc{L})$ where $V\subset X$ is a small tubular neighborhood of $L_1$, and $j'\colon V-L_1\ar X$ is the inclusion.

The colattice spectral sequence in this case is \emph{not} the long exact sequence above.
In fact its page ${}^{L}E^{**}_2$ is expressed in terms of $\mb{H}^*(L_1;i^*R^qj_*\mc{L})$ and 
$\mb{H}^*(L_1,L_0;\mc{L})$. It is especially useful when $i^* R^qj_*\mc{L}$ are local systems on the strata $L_0$. 
We will describe it in general in the next sections.

\subsection{A brief recap on homotopy limits and colimits}
Suppose $\mc{A}$ is a bicomplete abelian category 
(e.g. $\Sh_X$),
$P$ is a small category and $K\colon P\ar \mc{A}$ is a diagram of shape $P$.
Since $\mc{A}$ is closed under limits and colimits one has adjunctions: 
$$\colim(-)\colon \Fun(P,\mc{A})\ \substack{\lar\\ \lal}\ \mc{A}\colon \const_{-},$$
and
$$\const_{-}\colon  \mc{A}\ \substack{\lar\\ \lal}\ \Fun(P,\mc{A})\colon \prlim(-),$$
where $\const_{-}$ is the functor of constant diagram.
For a diagram $K$ with objects $K_t,t\in P$ we will often write 
$\colim(K),\colim(K,P)$ or $\colim(K_t,t\in P)$ when convenient.

It follows that $\colim(-)$ is right exact, while $\prlim(-)$ is left exact. 
Thus one can derive these functors to get $\mb{L}\colim\colon D(\Fun(P,\mc{A}))\ar D(\mc{A})$,
and similarly for $\mb{R}\prlim$.
From the model category perspective, in order to compute $\mb{L}\colim(K)$ one should replace $K$ 
by a cofibrant resolution $K'\ar K$ of the same shape and then evaluate $\colim(K')$.
For example, given two morphisms $f,g\colon A\ar B$, 
the coequalizer $\coeq(f,g):=\colim [A\substack{\lar\\ \lar}B]$
is equal to $\coeq(f-g,0)$, and if $f-g$ is injective, then $\coeq(f-g,0)=\coker(f-g)$. 
In general $\mb{L}\coeq(f,g)$ is equivalent to $\Cone[A\ar[f-g] B]$.
Similarly $\mb{R}\Eq(f,g)$ can be computed as $\Cone[A\ar[f-g]B][-1]$.

It is convenient to give another well-known description of these derived functors.
Recall that $\colim(K)$ is the coequalizer
$$\colim(K)=\colim\left[\bigoplus\limits_{x\ar x'\in P}K_x\substack{\lar\\\lar}\bigoplus\limits_{x\in P}K_x\right],$$
with respect to the morphisms induced by the projection and the composition along $x\ar x'$.
In fact there is a simplicial object given by the bar construction:
$$\sBar(K)_{\bullet}:=\left[\ldots \bigoplus\limits_{x\ar x'\ar x''}K_x
\substack{\lar\\\lal\\ \lar\\\lal\\ \lar}
\bigoplus\limits_{x\ar x'}K_x\substack{\lar\\\lal\\\lar}\bigoplus\limits_{x}K_x\right]\in \Fun(\Delta^{\op},\Ch(\mc{A})).$$
One can define $\hocolim(K)$ to be the normalized complex $N(\sBar(K)_{\bullet})\in \Ch(\mc{A})$;
it is parametrized by non degenerate paths (i.e.\ without the identity arrows between $x$'s).

Similarly $\prlim(K)$ is an equalizer and we have the cosimplical object
$$\sBar(K)^{\bullet}=
\left[\prod\limits_{x}K_x
\substack{\lar\\ \lal\\ \lar}
\prod\limits_{x'\ar x}K_{x}
\substack{\lar\\ \lal\\ \lar\\ \lal\\ \lar}\prod\limits_{x''\ar x'\ar x}K_x\ldots\right]\in \Fun(\Delta,\Ch(\mc{A})).$$
Define $\holim(K)=N(\sBar(K)^{\bullet})$.
It is a standard fact that on the derived level there are equivalences 
$\hocolim=\mb{L}\colim$ and $\holim=\mb{R}\prlim$.

\begin{exmpl}
	For a constant diagram $\const_A$ of shape $P$ we have
	$\hocolim(\const_A)\simeq A\otimes C_*(N(P))$ where $N(P)$ denotes the nerve of the category $P$ and $C_*(N(P))$ the chain complex of the simplicial set $N(P)$.
	Similarly, $\holim(\const_A)\simeq A\otimes C^*(N(P))$ where $C^*(N(P))$ is the corresponding cochain complex.
\end{exmpl}

In the particular case when $P$ is a poset one can interpret $\holim$ as follows.
The set of elements in $P$ admits a topology with the base formed by the sets $P_{\le x}$ 
(it is the smallest open containg $x\in L$).
Denote the corresponding (usually non-Hausdorff) topological space by $|P|$.
One can check that the functor of stalks $\Sh_{|P|}(\mc{A})\ar \Fun(P,\mc{A})$ is an equivalence of categories.
Under this equivalence we have $\Gamma(K)\simeq \prlim(K)\in \mc{A}$.
Recall that the Godement resolution for $K$ is a functorial cosimplicial sheaf with flabby components.
One can check directly that applying this cosimplicial resolution to $R\Gamma(K)$ 
we get $\sBar(K)^{\bullet}$.


\subsection{Lattice spectral sequence}
Fix a complex $\tilde{\mc{L}}\in \Ch(\Sh_X)$.
The sheaves $K_x:=(i_*Ri^!)_x \tilde{\mc{L}},x\in L$ form a diagram $K_{-}\colon L\ar \Sh(X)$ 
such that $K_1=\tilde{\mc{L}}$.
\begin{prop}
	There is a natural quasi-isomorphism 
	$$K:=\Cone[\hocolim_{x<1}K_x\ar K_1]\ar Rj_*j^* K_1.$$
\end{prop}
\begin{proof}
	Due to the existence of the Godement resolution 
	it is enough to prove the claim in the case 
	$K_1\in \Sh_X$ is a \emph{Godement sheaf}: 
	there is a sheaf $G$ such that for each open $V$ we have 
	$K_1(V)=\prod_{p\in V}G_p$.
	Since $K_1$ is flabby we can write $j_*j^*K_1=Rj_*j^*K_1$.
	For a Godement sheaf $K_1$ we call the stalk $G_p$ the \emph{value} of $K_1$ at $p$.
	One can write $K_x(V)=\prod_{p\in V\cap L_x}G_p\subset K_1(V)$, 
	this way $K_x$ are Godement sheaves too.
	We identify $j_* j^*K_1(V)=\prod_{p\in V-\cup_{x<1} L_x}G_p$ with a subsheaf of $K_1$
	with vanishing values at all $p\in \cup_{x<1}L_x$. 
	So for any $x\in L,p\in X$ the value of $K_x$ at $p$ is either $0$ 
	or is equal to the value of $K_1$ at $p$.
	
	Assume $x\in L$ is the lowest element such that $p\in L_x$.
	Then the values of $K_t$ and $K_1$ at $p$ are equal iff $t\ge x$.
	Using the bar construction one can show that 
	the values of $\hocolim_{t<1}K_t$ and $\hocolim_{x\le t<1}K_t$ at $p$ are equal
	to $G_p\otimes C_*(N[x,1))$.
	If $x<1$, then $[x,1)$ has a smallest element $x$, so $C_*(N[x,1))\simeq \mb{Z}$, hence
	the value of $\Cone[\hocolim_{x<1}K_x\ar K_1]$ at $p$ is zero.
	If $x=1$, then $N[x,1)$ is empty and the value of the cone at $p$ is the value of 
	$j_*j^*K_1=Rj_*j^*K$ at $p$.
	This proves the claim.
\end{proof}
Thus we consider $K$ as a resolution of $Rj_*j^*K_1$.
We define an increasing filtration by setting 
$F_r(K):=\Cone[\hocolim_{r(1)>r(x)\ge -r}K_x\ar K_1]$ for $r\ge-r(1)$,
and $F_{<-r(1)}(K):=0$.
\begin{rmrk}
	One can interpret $\Cone[\hocolim_{x<1}K_x\ar K_1]=\hocolim[\hocolim_{x<1}K_x\substack{\lar\\ \lar}K_1]$ 
	as a homotopy colimit over
	a diagram $K'_{-}$ of shape $L'$ where $L'$ is 
	obtained from $L$ by doubling all arrows $x<1$, and $K'$ is obtained by adding zero morphisms 
	to the diagram along $x<1$.
	The diagram $L'$ is not a poset, though it is directed by the rank function $r$. 
	Then $r$ defines a filtration on $\hocolim K'$, which coincides with the one given above.
\end{rmrk}
The \emph{lattice spectral sequence} ${}_{L}E_k$ is associated with the filtration $F_r(K)$. We have 
$${}_{L}E^{pq}_1=\mb{H}^{p+q}(X;\Cone[F_{-p-1}(K)\ar F_{-p}(K)]).$$
In order to describe this term let $\bar{C}_*(N(x,1))$ denote 
the reduced chain complex of the open interval $(x,1)\subset L$: 
if $(x,1)\neq \emptyset$ it is given by the natural augmentation by adding $\mb{Z}$ in cohomological degree $1$
(i.e.\ by adding a $(-1)$-simplex);
otherwise it will be convenient to set $\bar{C}_*(\emptyset)=\mb{Z}[-2]$.
\begin{prop}
	For each $r$ there is an equivalence
	$$\Cone[F_{r-1}(K)\ar F_r(K)]\simeq \bigoplus\limits_{r(x)=-r}K_x\otimes \bar{C}_*(N(x,1))[2].$$
\end{prop}
\begin{proof}
	If $r=-r(1)$ then $\Cone[F_{r-1}(K)\ar F_r(K)]=K_1$, and if $r<-r(1)$ then 
	the both parts are trivial 
	in accordance with the assertion.
	Suppose $r\ge -r(1)$ and
	let $\delta_x\colon P\ar \Ab$ denote the diagram with $\mb{Z}$ at $x\in L$ and zero otherwise.
	Consider $K_t\otimes (\delta_x)_t$ as a diagram of the shape 
	$\{t\mid r(1)>r(t)\ge -r\}\subset L$.
	Using the bar construction it is not difficult to see that 
	$$\Cone[F_{r-1}(K)\ar F_r(K)]\simeq 
	\bigoplus\limits_{r(x)=-r}\hocolim_{x\le t<1}K_t\otimes (\delta_x)_t[1],$$
	%On the other hand 
	%$$\hocolim_{r(t)\le -r,t<1} K_t\otimes (\delta_x)_t=\hocolim_{t\le x}K_t\otimes \delta_x$$
	%computed by means of the bar construction 
	while $\hocolim_{x\le t<1}K_t\otimes (\delta_x)_t$ for a given $x$ is equal to
\begin{equation}\label{simpl_lattice_spec_seq}
\left[\ldots \bigoplus\limits_{x\ar x'\ar x''}F_x
\substack{\lar\\\lal\\ \lar\\\lal\\ \lar}\bigoplus\limits_{x\ar x'}K_x 
	\substack{\lar\\\lal\\ \lar\\}K_x\right],
\end{equation}
	where all $x'$'s and $x''$'s etc.\ run through $[x,1)\subset L$.
	One can check that the normalization of~\eqref{simpl_lattice_spec_seq} coincides with
	$K_x\otimes \bar{C}_*(N(x,1))[1]$, which concludes the proof.
\end{proof}

Recall that $(L,\le)$ is the intersection poset of an arrangement in $X$, and $\tilde{\mc{L}}\in \Ch(\Sh_X)$.
As corollary we obtain an expression for the lattice spectral sequence:
\begin{thrm}[Tosteson \cite{To}, Petersen \cite{Petersen}]
	There is a spectral sequence 
	with the first term equal to
	$${}_{L}E^{pq}_1=
	\bigoplus\limits_{r(x)=p}
	\mb{H}^{p+q}_{L_x}(X;\tilde{\mc{L}}\otimes \bar{C}_*(N(x,1))[2])$$
	converging to $\mb{H}^*(U;j^*\tilde{\mc{L}})$.
\end{thrm}
\begin{rmrk}
	By the work of Yuzvinsky \cite{YuzAtomic}, 
	$\bar{C}_*(N(x,1))[2]$ is naturally equivalent
	to the (relative) atomic complex $\mc{D}(L)_x$ of $L$ 
	(see \ref{GorMac}).
\end{rmrk}

\subsection{The colattice spectral sequence}
In the setup of the previous subsection we construct another spectral sequence associated with 
the complex $\mc{L}\in \Ch(\Sh_U)$ and
the intersection poset $(L,\le)$.
The sheaves $K^x:=(i_*i^*)_x Rj_*\mc{L}$ form a diagram $L^{\op}\ar \Ch(\Sh_X)$ with the
morphisms induced by the restrictions along the inclusions $L_x\ar L_y,x\le y$.
The initial (smallest) element is $K^1=Rj_*\mc{L}$.
Set $X_{\le r}:=\cup_{r(x)\le r}L_x$, and let $i_{\le r}\colon X_{\le r}\ar X$ be the corresponding inclusion.
First we will construct a decreasing filtration $F^r(K^1)$ of $K^1$ using the filtration $X_{\le r}$ of $X$.

The following Proposition is not necessary for what follows, but we decided to include it in order to make a comparison with the previous construction more transparent.
\begin{prop}
	There is a natural quasi-isomorphism
	$(i_*i^*)_{\le r}K^1\ar \holim_{r(t)\le r}K^t.$
\end{prop}
\begin{proof}
	Let $M=\{t\in L\mid r(t)\le r\}^{\op}\subset L^{\op}$.
	By definition, the stalk $K^x_p$ at $p\in X$ is equal to
	$K^1_p$ if $p\in L_x\subset X$ and is zero otherwise.
	On the other hand, $\holim(K^t,t\in M)_p\simeq \holim(K^t_p,t\in M)$, 
	since taking the stalk is an exact functor.
	It remains to show that the natural morphism
	$$(i_*i^*)_{\le r}K^1_p\ar \holim(K^t_p,t\in M)$$
	of stalks is an equivalence for all $p\in X$.
	Let $y\in L$ be the minimal element such that $p\in L_y$.
	If $r(y)\not\le r$, then $p\not\in X_{\le r}$ and 
	the stalks are trivial.
	
	Suppose $r(y)\le r$.
	Consider the subposets 
	$M':=\{t\in M\mid y\le t\}$ and 
	$\bar{M'}:=\{t\in M\mid t\not\in M'\}$ of $M$.
	Then $K^t_p\neq 0$ implies $t\in M'$. 
	For all $t\in M'$ we have $K^t_p\simeq K^1_p$, and
	hence $\holim(K^t,t\in M')\simeq K^1_p$ since $y$ is initial in $M'$.

	On the other hand,
	$\sBar(K^t_p,t\in M')^{\bullet}\ar \sBar(K^t_p,t\in M)^{\bullet}$ is an inclusion 
	with the quotient isomorphic to $\sBar(0,t\in \bar{M'})^{\bullet}$, which is trivial.
	Hence $$(i_*i^*)_{\le r}K^1_p\simeq K^1_p\simeq \holim(K^t_p,t\in M')\ar \holim(K^t_p,t\in M)$$ 
	is a chain of equivalences.
	This proves the claim.
\end{proof}

Define a filtration of $K_1$ by setting
$$F'^{r}(K^1)=\Cone[K^1\ar (i_*i^*)_{<r}K^1][-1].$$
Let $j_x\colon L_x-\cup_{y<x}L_y\lar X$ be the inclusion of the stratum corresponding to $L_x$.
\begin{prop}
	There is an equivalence
	$$\Cone[F'^{r+1}(K^1)\ar F'^r(K^1)]\simeq \oplus_{r(x)=r}(j_!j^*)_x K^1.$$
\end{prop}
\begin{proof}
	The left hand side is equivalent to $\Cone[(i_*i^*)_{\le r}K^1\ar (i_*i^*)_{<r}K^1][-1]$.
	On the other hand we have a triangle
	$$(j_!j^*)_{r}\ar (i_*i^*)_{\le r}\ar (i_*i^*)_{<r}\ar (j_!j^*)_r[1]$$
	where $j_r\colon X_{\le r}- X_{<r}\lar X$ is the inclusion of a disjoint union of strata; it is equal to 
	$\sqcup_{r(x)=r}j_x$.
	Hence $\Cone[F'^{r+1}(K^1)\ar F'^r(K^1)]\simeq (j_!j^*)_r K^1$.
\end{proof}

Recall that $K^1=Rj_*\mc{L}$.
Let $({}_{F'}\mathcal{E}_k,d_k)$ denotes the sheaf spectral sequence for the filtration $F'$ on $Rj_*\mc{L}$.
Here by the definition the complex ${}_{F'}\mc{E}^{p,*}_0$ is equal to 
$\Gr^r_{F'}[r]:=\Cone[F'^{r+1}\ar F'^r][r]$,
so
\begin{lemma}
	We have
$${}_{F'}\mc{E}^{pq}_1=\oplus_{r(x)=p}(j_!j^*)_x R^{p+q}j_*\mc{L}\in \Ch(\Sh_X).$$
Moreover $d_{\ge 1}=0$, i.e. ${}_{F'}\mc{E}_1={}_{F'}\mc{E}_{\infty}$.
\end{lemma}
\begin{proof}
	The expression for ${}_{F'}\mc{E}^{pq}_1$ follows from the exactness of $j_!$ and $j^*$.
	The last assertion is evident since the terms $\mc{E}^{pq}_k,k\ge 1$ are ordinary sheaves 
	supported on disjoint strata while $d_k,k\ge 1$ increases the value of~$r$.
\end{proof}
It is convenient to consider Deligne's d\'ecalage filtration $\Dec(F')$.
Recall (see Proposition~\ref{prop:decalage_ss}) that there is a natural morphism 
$${}_{\Dec(F')}\mc{E}^{pq}_0\ar {}_{F'}\mc{E}^{2p+q,-p}_1,$$
which is a quasi-isomorphism of the underlying complexes of sheaves.
By the previous lemma the column $({}_{\Dec(F')}\mc{E}^{p,*}_0,d_0)=\Gr^p_{\Dec(F')}[p]$ is quasi-isomorphic to 
$$\bigoplus\limits_{i} {}_{F'}\mc{E}^{2p+i,-p}_1[-i]=
\bigoplus\limits_i \bigoplus\limits_{r(x)=2p+i}(j_!j^*)_x R^{p+i}j_*\mc{L}[-i]=
\bigoplus\limits_x (j_!j^*)_x R^{r(x)-p}j_*\mc{L}[2p-r(x)]$$ with trivial differential.
Hence the usual hypercohomology spectral sequence of $(Rj_*\mc{L},\Dec(F'))$ is given by
$${}_{\Dec(F')}E^{pq}_1=\mb{H}^{q}(X;\Gr^p_{\Dec(F')}[p])\simeq
\bigoplus\limits_x \mb{H}^{q+2p-r(x)}(X;(j_!j^*)_x R^{r(x)-p}j_*\mc{L}),$$
and converges $\mb{H}^{p+q}(Rj_*\mc{L})$.
By using d\'ecalage again we recover the colattice spectral sequence:
\begin{thrm}[Denham-Suciu-Yuzvinsky \cite{DSY}]
	There is a spectral sequence ${}^{L}E^{pq}_k$ 
	converging to $\mb{H}^{p+q}(U;\mc{L})$ such that
	$${}^{L}E^{ab}_2={}_{\Dec(F')}E^{-b,a+2b}_1=
	\bigoplus_{x\in L}\mb{H}^{a-r(x)}(X;(j_!j^*)_x R^{b+r(x)}j_*\mc{L}).$$
\end{thrm}
\resumetoc


